Affordance as general value function: A computational model

General value functions (GVFs) in the reinforcement learning (RL) literature are long-term predictive summaries of the outcomes of agents following specific policies in the environment. Affordances as perceived action possibilities with specific valence may be cast into predicted policy-relative goodness and modelled as GVFs. A systematic explication of this connection shows that GVFs and especially their deep learning embodiments (1) realize affordance prediction as a form of direct perception, (2) illuminate the fundamental connection between action and perception in affordance, and (3) offer a scalable way to learn affordances using RL methods. Through an extensive review of existing literature on GVF applications and representative affordance research in robotics, we demonstrate that GVFs provide the right framework for learning affordances in real-world applications. In addition, we highlight a few new avenues of research opened up by the perspective of "affordance as GVF", including using GVFs for orchestrating complex behaviors.

==> applications.tex <==
\section{Applications of GVFs}
% There are a small but growing number of examples where GVFs are being applied to real-world problems including (1) prosthetic arms \citep{pilarski2013} \citep{edwards2016}, (2) aiding mammals with partial paralysis \citep{dalrymple2020pavlovian}, (3) industrial automation \citep{gunther2016}, (4) robots \citep{sutton2011} \citep{modayil2012} and (5) autonomous driving \citep{graves2019a} \citep{graves2020}.
While GVFs have not been broadly adopted in real-world applications,
there are a small but growing number of examples where they are applied to real-world problems including (1) robots \citep{sutton2011, modayil2012}, (2) prosthetic arms \citep{pilarski2013, edwards2016}, (3) aiding mammals with partial paralysis \citep{dalrymple2020pavlovian}, (4) industrial automation \citep{gunther2016} and (5) autonomous driving \citep{graves2019a, graves2020}.
In this section, we introduce such applications of GVFs and discuss how they relate to affordances.

\subsection{Robotics}
GVFs were first introduced by \citet{sutton2011} as a way to learn predictions about sensor readings in a factored and modular way.
% They learn the relationship about the sensors and actuators from unsupervised experience.
They learn the relationship between current sensor readings and future readings in an unsupervised way, while taking the actuators into account.
To demonstrate the idea, \citet{sutton2011} conducted experiments on the Critterbot robotic platform and predicted (1) time to obstacle with infrared sensors, and (2) time to stop on different types of floor materials. 
They also presented a way to learn \textit{off policy} these future sensor readings as a proof-of-concept. 
In addition, they demonstrated how several of the off-policy predictions can be used in various policies by maximizing infrared readings, maximizing magnetometer readings, maximizing velocity through spinning actions, and maximizing light sensor readings.
In the last case, the agent successfully sought sources of light by maximizing predicted light sensor readings.
It is important to note that in these experiments, the agent was following random policies while it learned predictions concerning goal-directed behaviour with GVFs.
This demonstrates how GVF-based predictions can represent the outcome of goal-driven behaviour, even when the behaviour experienced during learning was different.
% In all cases, the agent was learning the predictions from entirely random behavior policies and demonstrated how each prediction could be used to generate goal-directed behavior.
% This was the first step at demonstrating that each GVF prediction can represent the outcome of a goal for the agent.
\citet{sutton2011} suggest that a ``horde'' of such predictions can thus form bits of knowledge that can be used to solve more complex tasks. With these kinds of GVF predictions, one can represent the world more compactly and make more informative decisions---based on the relationship between states, outcomes, and behaviour---than history alone allows \citep{schaul2013}.

The connection to psychology was a motivating factor in early GVF research.
% In \citep{modayil2012}, authors drew a connection between GVF predictions and nexting \citep{gilbert2003} which is a term referring to making simple, short-term, personal predictions.
\citet{modayil2012}, for example, drew a connection between GVF predictions and \textit{nexting} \citep{gilbert2003}, which is the phenomenon of a person simultaneously making a large number of predictions about general environment conditions on a short timescale.
They experiment on the Critterbot and evaluated the accuracy of learning predictions of the robot's light sensor.
They concluded that GVFs are an effective and practical way to learn many nexting predictions in parallel.

\citet{abeyruwan2014} describe an interesting use of GVFs for selecting role assignments of a team of agents in the RoboCup 3D simulation.
An agent can choose one of a fixed number of 13 ``roles'' on the field.
It must predict the value and uniqueness of its role among all other agents without communicating its role to the other agents on the team.
The roles that are predicted to be unique represent action possibilities available to the agent.
Thus, the prediction of uniqueness may be interpreted as a kind of affordance prediction to encourage coordinated team play without verbal communication in the simulated RoboCup 3D soccer game.

\subsection{Rehabilitation}
Predictions and predictive knowledge have been argued to be important parts of intelligent systems, especially when they are meant to interact with humans \citep{pilarski2019learned}. An important application domain for such an interactive relationship is rehabilitation. Here, an intelligent system can either be a prosthetic, robotic device \citep{edwards2016} or an algorithm that is directly interacting with the biological system \citep{dalrymple2020pavlovian}.

\noindent
\textbf{Prosthetic Arms:} 
Recent research has shown the benefit of predictions when used for prosthetic limbs \citep{pilarski2013, sherstan2014, gunther2018}.  Since computation for GVFs scales linearly with the number of predictions, when combined with (linear) function approximation they are a natural choice to create predictive knowledge for systems with limited hardware capabilities, such as prosthetic limbs. 
As \citet{sherstan2014} have shown, an abundant number of GVFs can be learned and maintained with reasonable computational resources that would allow these techniques to be used in mobile devices.
Such GVF-based predictions have been demonstrated to be useful for prosthetic limbs in two ways. First, they allow better communication between the prosthesis and its wearer \citep{edwards2016}. Second, they contain and generate data that is a useful source of information \citep{sherstan2014, gunther2018}. From the affordance perspective, these advantages make the prosthetic devices easier to use because the GVF-based predictions are learned in an ecological context and through an interactive process wherein the devices are actively engaged. 
If these GVFs can in fact be used as affordances, they would allow a paradigm shift for amputees: prosthetic devices could be used as intuitively as natural limbs---by deciding what the wearer wants its device to do instead of consciously moving it into a position.

\begin{figure}[!t]
\centering
\includegraphics[width = \columnwidth]{mpl.eps}
\caption{The Modular Prosthetic Limb (MPL), a robot arm with many degrees of freedom and sensors used for research in prosthetic limbs \citep{gunther2020examining}.}
\label{fig:mpl}
\end{figure}

\citet{edwards2016} used a GVF-based prediction to decide the order in which the prosthetic limb joints are activated during a pick-and-place task.
The order of joints that is required to complete the task is predicted. Availability of such a prediction spares the amputee from having to intently switch repeatedly among joints that are not required to move at the same time.
It furnishes the prosthetic limb with the correct choice for the joint to activate, which arguably corresponds to the affordance for motion of the limb as a whole, and thereby allows the amputee to achieve their motion goal faster and easier.
% \subsection{Prosthetic Arms}
% Predictions and predictive knowledge have been argued to be important parts of intelligent systems, among them prosthetic limbs \citep{pilarski2013}, \citep{sherstan2014}, \citep{gunther2018}.
% Furthermore, predictions can be used in a layered way to make predictions of predictions, resulting in more complex knowledge \citep{schaul2013}.
% This approach has demonstrated its merits especially in partially observable environments \citep{schlegel2018}, \citep{schaul2013}.

% As GVFs scale linearly, when combined with (linear) function approximation they are a natural choice to create predictive knowledge.
% As \citep{sherstan2014} have shown in their paper, an abundant number of GVFs can be learned and maintained with reasonable computational resources that would allow these techniques to be used in mobile devices, such as prosthetic limbs.
% Such GVF-based predictive approaches have demonstrated to be useful for prosthetic limbs twofold---they allow better communication between the prosthesis and its wearer \citep{edwards2016} and they furthermore contain and generate data that is a useful source of information \citep{sherstan2014}, \citep{gunther2018}.

% \citep{edwards2016} used a GVF-based prediction to decide the order in which the prosthetic limb joints are activated during a pick and place task.
% The prediction learns the order of joints that are required to complete the task, thus sparing the amputee to switch repeatedly among joints that are not required to move at the same time.
% Here, the GVF-based prediction directly corresponds to the affordance.
% It provides the prosthetic limb with the correct choice for the joint to activate, thus enabling the amputee to achieve the goal faster and easier.

In addition to providing predictions, GVFs can furthermore serve as additional sources of information.
\citet{gunther2018} investigate the relationship of errors that occur during learning from surprising external signals.
They use the \textit{unexpected demon error} (UDE) \citep{awhite2015} as a measure of surprise.
As in \citep{sutton2011}, the term \textit{demon} here refers to a single GVF.
\citet{gunther2018} show how movements that are not expected give rise to a high UDE, or surprise, during the functioning of a prosthetic limb.
The relationship between surprise and affordances is still ongoing research, but one can imagine how sensory information that triggers surprise may be directly related to actions. One such example would be an unfamiliar movement with a prosthetic arm that occurs while learning a new task. Such a surprise informs the learning agent about the need for learning, which can be accommodated by increasing the learning rate. Another example could be active exploration that is triggered by surprise. A prosthetic arm that is surprised about its failing to grasp an object would actively explore the shape of the unfamiliar object, thus learning its affordances and improving the handling of it.


\noindent
\textbf{Aiding Mammals with Partial Paralysis: } \citet{dalrymple2020pavlovian} used GVFs in a very unique way to directly interface with living mammals. Unlike in the previous examples, where the predictions provide a better interface between the amputee and the prosthetic, the predictions are used to directly control a limb of mammals.
In their paper they developed a predictive control strategy---utilizing GVFs---to enable cats with spinal cord injury to walk.
% produce an alternating walking pattern in cats with spinal cord injury.
To this end, eight cats were anaesthetized and each placed in a sling. Data for learning was gathered by manually moving the cat's left hind-limb in order to create a normal moving pattern that could then be reproduced for the cat's right hind-limb. Two different control strategies were tested: one that utilized simple thresholds and one that used learned GVF-based predictions. 
The GVF-based approach used \textit{Pavlovian Control} for controlling the limb, wherein stimulation of the cat's limb was directly linked to the predictions made by the GVFs, similar to a conditioned response to an anticipation. The cumulants for the three predictions were \textit{unloading}, \textit{ground reaction force} and \textit{angular velocity}. The ground reaction force and angular velocity for both hind-limbs were used as measurements to inform the GVFs, i.e. to construct the state. 

\citet{dalrymple2020pavlovian} found that the GVFs learned the walking pattern in no more than four steps and that the learned predictions were transferable between different humans training the movement and different cats, and furthermore were able to recover from mistakes during demonstration with the left hind-limb.

The GVFs here arguably represent affordances of the cat's own body---as the left hind-limb engages a movement, the GVFs provide the right hind-limb with the action to complete the movement pattern, thus enabling a paralyzed cat to walk.

\subsection{Industrial Automation}
GVFs have been successfully applied in industrial control problems that are too complex to be sufficiently measured or observed and thus have been historically modelled as open-loop processes. Using machine learning---GVFs in particular---these open-loop processes can potentially be transformed into closed-loop processes, allowing them to run reliably without the need for human supervision.

\begin{figure}
    \centering
    \includegraphics[width = \columnwidth]{figures/architecture.eps}
    \caption{Control architecture, used for industrial laser welding. The GVF predictions---produced by the ``process knowledge'' block---are informed by features from the sensor data and then used for process control \citep{gunther2016}.
    }
    \label{fig:my_label}
\end{figure}

An example in question is industrial laser welding.
Due to lack of appropriate sensors, the quality of welding cannot be measured while the process is running, resulting in the need for time- and labour-intensive quality control. \citet{gunther2016} demonstrate how GVFs can be used to predict the quality of the welding seam from a camera using deep learning.
The GVFs therefore provide a synthesized feedback signal. This feedback signal can then be used to inform control decisions, forming a closed control loop.

Welding quality is here measured on a scale from one to four, according to the international norm for laser welding (ISO 13919-1:1996).
\citet{gunther2016} showed the first application that combined GVFs with deep learning.
A deep auto-encoder is used to extract features from in-line welding images online.
These features are then paired with additional sensor data from photodiodes and serve as input for a linear function approximator to provide the state for the GVFs.

The performance was evaluated on real-world data, collected in a laser laboratory.
By combining deep learning with GVFs, the approach resulted in a mapping that is invariant to rotation, translation and scaling and performed with high accuracy (F score of 0.928) \citep{gunther2018machine}.
Furthermore, the GVFs enable anticipation of changes in the welding seam quality before they occurred, allowing for predictive control.

In addition, the GVF output was eventually used in a control setting to adjust the laser intensity.
The controller was trained and evaluated in simulation and demonstrated promising results wherein the correct welding depth is achieved.
% The controller of laser intensity is trained using actor-critic methods in RL to maximize total discounted reward as predicted by the GVF output.
The effective use of GVF predictions---predicted weld quality in this example---to support the construction and learning of effective control policies supports our general thesis that GVF predictions represent affordances---quality for the action of welding here in this example.

\subsection{Autonomous Driving}
Autonomous driving is a growing field of research for deep reinforcement learning that tests the limits of modern robotics applications.
Recently, GVFs have been demonstrated to in adaptive cruise control \citep{graves2019a} and vision-based steering \citep{graves2020}.
These works highlight the promise for broader application of GVF predictions to autonomous driving.

\citet{graves2019a} trained GAVFs that predicted future safety, speed, and closeness to the desired target speed for a fixed target policy $\tau$.
The target policy $\tau$ was a normal distribution centered on the previous action.
The GAVFs, which are a function of state $s$ and action $a$, were used as a partial model to predict the desired outcomes of safety and speed when following the target policy beginning with action $a$.
For example, the safety prediction answered the following question: ``what will my safety be if I take action $a$ and follow similar actions according to the target policy there after.''
Many predictions of safety and speed were made for a number of different possible actions to decide the best next action that satisfies the criteria of being safe while cruising at the desired target speed.
These kinds of predictive questions are affordances that permit an agent to plan by inferring a good policy from a limited number of hypothetical ``what-if'' predictions.
The planning is constrained to the policies of the GAVFs and thus does not require extensive search by iterating next step models.

\citet{graves2019a} showed that a limited number of predictions could be used to control both a real robot and an autonomous vehicle from a high dimensional LIDAR sensor data stream with performance competitive with existing solutions.
It was shown that driving with predictions from high dimensional raw data streams is both scalable and computationally efficient compared to classical planning approaches where searching for the best action possibility out of $n$ available action possibilities is linear in $n$.
On the other hand, traditional planning methods search for the best action sequence upto the desired temporal horizon.

This works was extended to the more complex task of driving a vehicle from vision-based sensors \citep{graves2020}.  GVFs were used to steer a vehicle with just a front-facing camera by learning a limited number of predictions of the future lane centeredness and angle offset with the road over multiple time horizons.
It was found that predicting over multiple time horizons was crucial for achieving excellent performance and generalization to unseen roads including roads with damaged lane markings.
Not only was the robot able to steer well on unseen roads but it was also able to slow down for tight corners.
In addition, the authors showed how both the predictions and final steering policy could be learned directly from data collected in the real-world thereby bypassing the sim-to-real issues that are typical when applying RL to the real-world.

\begin{figure}
    \centering
    \includegraphics[width=0.45\textwidth]{figures/jackal_robot_visual_steering_annotated.eps}
    \caption{Jackal robot driving on a visually challenging road using GVFs as a predictive representation of state}
    \label{fig_jackal_robot_visual_steering}
\end{figure}
\begin{figure}
    \centering
    \includegraphics[width=0.45\textwidth]{figures/temporal_horizon_steering.eps}
    \caption{Depiction of the different temporal horizons of the GVF predictions for driving with GVFs}
    \label{fig_visual_steering_temporal_horizon}
\end{figure}
The lane centeredness and road offset predictions can be viewed as affordances under the policy of driving with approximately constant steering and speed actions until an out of lane event occurs.
By predicting the effects over different temporal horizons on future lane centeredness and angle offset with the road, the controller had enough information to decide pro-active corrective measures to keep the vehicle centered in the lane.
Eight predictions over four time scales were learned as depicted in Figure \ref{fig_visual_steering_temporal_horizon}.
The predictions formed a predictive representation that served as an intermediate layer in representing the state, based on which an RL agent learns to steer.
The RL agent was trained using only this intermediate predictive layer and was able to learn quickly, achieving much better control that generalized better to unseen roads than end-to-end RL approaches.
The benefits reported include better learning, smoother control and better generalization to unseen roads \citep{graves2020}.
These advantages make for safe, fast, and comfortable autonomous driving.

\subsection{Discussion}
Our survey of the existing literature on the various applications of GVFs to real-world problems revealed common themes that are consistent with our proposal that affordances should be modelled by GVFs.
While many works focused on learning real-world predictive knowledge without direct ways to use that knowledge \citep{sutton2011, modayil2012, sherstan2014, awhite2015, gunther2018}, a growing number of applications directly demonstrate how the predictions can be used in real-world applications: (1) human-in-the-loop control with predictive knowledge \citep{pilarski2013, edwards2016}, (2) closed-loop control with predictive representations and predictive feedback \citep{gunther2016, gunther2018machine, graves2020}, (3) Pavlovian control with hand-engineered rules based on predictions \citep{dalrymple2020pavlovian, graves2019a}, and (4) role assignment of agents in multi-agent problems \citep{abeyruwan2014}.
The first approach of human-in-the-loop control demonstrates that humans can control prosthetic limbs more effectively when their affordances are communicated through GVF predictions.
The second approach demonstrates that closed-loop control with an RL-based policy can be achieved using GVF predictions that correspond to affordances as the normally missing feedback signal.
It allows realization of high-performance behavior that can be challenging to achieve without predictions, in a way that is reminiscent of the situation with batting in baseball \citep{epstein2013sports}.
The third approach, called Pavlovian control, demonstrates how GVF predictions can be linked with simple engineered control rules to achieve intelligent behavior.
The advantage of Pavlovian control with the right predictions is that often simple controllers can be easily designed and tuned for good performance.
Finally, the fourth approach of role assignment demonstrates potential utility of GVF predictions in multi-agent problems.


==> extra.tex <==
\subsection{Affordances as Predictive State Representations}
% TODO: Dan - completely rewrite this section to planning with Affordances (or GVFs or something similar)
% TODO: Dan - Figure 1 is not all that useful.  Some other drawing showing GVFs as a way to plan will be more useful (tree search vs GVF-based planning)
The connection between GVF predictions and affordances is not immediately obvious; the purpose of this work is highlight this connection and ask important research questions on the future direction of GVFs and affordance.
Affordances are directly perceived action possibilities \cite{zech2017}.
We claim that action possibilities, in the Gibson sense, are equivalent to options in reinforcement learning \cite{sutton1999}.
Recall that an option is defined as a tuple $(I, \gamma, \tau)$.
The available actions to the agent given state $s$ is described by the initiation set $I(s) \subset S$.
The policy and termination of the option $o \in O$ is given by $\tau$ and $\gamma$ respectively, where $O$ is the set of options available to the agent.
Therefore, an option provides a mathematical framework to describe action possibilities in affordance.
A GVF described by a cumulant $c$ and option $o$ predicts the long-term outcome of an option (or action possibility) on the cumulant when executing the option.

However, action possibilities are not enough:  how does one use them to plan and control the agent?
Exploitation of affordances is an important problem that requires prediction, planning and action selection \cite{zech2017}.
One published advantage with GVFs is the suitability to representing predictive state representations (PSRs) where representations have been shown to be both compact and general compared to using history alone, cf \cite{rafols2005} \cite{schlegel2018} \cite{schaul2013}.
Figure \ref{fig_affordances} shows a depiction of the different elements required to describe a predictive state representation with GVFs, or forecasts as referred to in \cite{schaul2013}.
Authors in \cite{schaul2013} in particular demonstrate a clear advantage in generalization abilities when using GVF forecasts to represent state over classical PSR approaches.
\cite{graves2019a} and \cite{graves2020} demonstrate how GVFs can be used to form a predictive state representation in autonomous driving for adaptive cruise control and steering from images, respectively.
%TODO steering reference - make sure it's posted online!

\begin{figure}
\centering
\includegraphics[width=12cm]{affordances.eps}
\caption{Affordances can be used to construct a predictive state representation using GVFs.  1) options are used to define the space of action possibilities given the current state.  2) cumulants define what to predict.  3) GVFs define the space of affordances.  4)  GVF predictions form a predictive state representation (PSR)}
\label{fig_affordances}
\end{figure}

We formalize affordances $A$ as the tuple $(O,C,\Omega)$, where $O$ is the set of all options available to the agent, $C$ is the set of all cumulants that can be observed in the environment, and $\Omega$ defines the set of all predictive questions.  $\omega \in \Omega$ is given by the tuple $(o,c,V^{\tau}_{c})$ with $o \in O$, $c \in C$ and $V^{\tau}_{c}$ estimating the value of the GVF following policy $\tau$ from option $o$ with cumulant $c$ is in \eqref{eq_gvf}.
The GVFs for each predictive question produce a vector that describes future of the robot which we denote as $\upsilon \in \Upsilon$.
It may be desirable for $\upsilon$ to satisfy the Markov property such that $\upsilon_{t+1}$ only depends on the current $\upsilon_{t}$ and action taken $a_{t}$, i.e. $p(\upsilon_{t+1}|\upsilon_{t},a_{t})=p(\upsilon_{t+1}|\upsilon_{t},a_{t},\upsilon_{t-1},a_{t-1},...,a_{0},\upsilon_{0})$.
If the Markov property is satisfied, then we say $\upsilon$ is a predictive state representation allowing for any number of techniques to be used to solve MDPs with this predictive representation including RL.

While there are definite advantages to predictive state representations with GVFs, such as those observed in \cite{schaul2013}, there are still many challenges to overcome including how to choose good predictive questions that represent the state of the agent.

In summary, GVFs make it possible to build predictive state representations on action possibilities (ie options).
This predictive representation describes outcomes of all the affordances available to an agent, filtered by the initiation set $I$ for each option (i.e. action possibility) for the current state of the agent.
However, what do with the predictions is still an open problem of research.
We suggest some approaches in the next section.

\subsection{Behavior Affording Behavior with GVFs}
% TODO: Dan - this should not be in the body -> create a new section on extending GVFs to include "spatial distributed predictions"
% TODO: Dan - rewrite this, condensing the content to a small section highlighting how GVFs provide a way to predict the success of policies that bring the agent into the a region of space that successfully predicts the success of another policy (prediction of another prediction)
% TODO: Dan - finally connect this with Behavior affording behavior concept instead of introducing it as this
Behavior affording behavior was coined by Gibson as a way to describe how some actions permit other actions to become available \cite{zech2017} \cite{gibson1979}.
One complaint about GVFs as a computational model of affordance is that they do not offer a way to ground affordances spatially to objects.
We argue that this is not necessary if we define objects by the kinds of interactions that we can make with them.
For example, a chair affords sitting; we argue that the object is a chair \textit{because} it affords sitting rather than the object is a chair \textit{therefore} it affords sitting.
This subtle distinction is important for highlighting that learning behavior that affords behavior is critical for computational models of affordance that do not explicitly detect objects through means of classification.
Using the chair example, the action of sitting may not be available without first finding a chair, walking over to it and then sitting.
This can be accomplished by executing a skill of finding a state that allows one to sit where we emphasize that detecting and classifying the object as a chair is not strictly necessary.
GVFs provide a way to learn behavior affording behavior which we will formalize here; however, unlike previous works with GVFs that do not consider the initiation set of the underlying option associated with a GVF prediction, we must consider the initiation set and assume it is a subset of the state space rather than equal to the entire state space.

Recall that a GVF is described by an option $o$ and a cumulant $c$ and the option is described by an initiation set $I$, policy $\tau$ and termination function $\gamma$.
We assume that the initiation set is a subset of the state space, i.e. $I \subset S$.
Note that it is common to assume the initiation set is equal to the state space; however, this approach will not lead to behavior affording behavior since the option is available in all states!
We can say that an option $o_1$ affords another option $o_2$ if the policy $\tau_2$ of option $o_2$ seeks terminal states that are in the initiation set $I_1$ of option $o_1$.
One way to explicitly accomplish this is by defining a control GVF $G_1$ with reward\footnote{Because this is a control GVF, the cumulant is usually referred to as reward instead of cumulant.} $c_1=1$ when $s \in I_2$ otherwise $c_1=0$.
The policy $\tau$ of the control GVF maximizes future accumulated reward.

As an example, suppose we have an option $o_\text{sit}$ which is not available to the agent, i.e. current state $s \not\in I_\text{sit}$.
We can define another option $o_\text{find}$ which aims to make the option $o_\text{sit}$ available to the agent.
One way to do this is to define a control GVF $G_\text{find}$ where the cumulant $c=1$ and termination $\gamma=0$ when in a state where $s \in I_\text{sit}$ and otherwise $c=0$ and $\gamma>0$.
Because this GVF is a control prediction, the cumulant is also the reward for an MDP and ($\tau_\text{find},\gamma_\text{find}, I_\text{find}$) defines an option $o_\text{find}$ that maximizes future accumulated reward.
However, this doesn't allow the agent to be selective about possible places to sit by the level of comfort.
We can define a GVF $G^\text{comfort}_\text{sit}$ with option $o_\text{sit}$ and cumulant $c$ equal to some measure of comfort when sitting; this GVF predicts the comfort level of sitting.
However, $o_\text{sit}$ is not available to the agent and thus $G^\text{comfort}_\text{sit}$ should predict low comfort; we can redefine the reward of $G_\text{find}$ to be $c=G^\text{find}_\text{sit}$ and termination $\gamma=0$ when in a state where $s \in I_\text{sit}$ and otherwise $c=0$ and $\gamma>0$.
In this way, GVFs and options provide a way to formally describe behavior that affords behavior.
Of course, learning the options, including the initiation set which has been largely ignored in the literature, is still a challenging problem; however, RL and GVFs in particular provide a theoretically grounded framework to build upon and discover new learning algorithms.

\subsection{Planning and Control with GVF Predictions}
% TODO: Dan - this section is irrelevant or unimportant as written  It's better to instead simply focus on GVFs as a way to enhance state representation for an agent and pull in predictive state representation literature.
For each option $o \in O$, there is a plan, or policy, that can be executed by the agent.
The set of GVF predictions corresponding to option $o$ describes the effect of that plan.
In this section, we equate a plan to an option in RL where the outcome of that plan is described by the GVF prediction.
Note that the effect of the plan may be multi-dimensional and have many effects, described by many cumulants.
The set of predictions $\Omega$ described by affordances $A$ thus considers all possible plans an agent could take.
A control algorithm can choose a plan to execute based on the predicted outcome of each plan by knowing $\upsilon$.

We see two approaches to achieving control:

\begin{itemize}
\item utilize the options framework to sequentially choose options that maximize accumulated reward
\item learn a policy that maximizes accumulated reward in a modified MDP $M^{\Upsilon}$ where $\Upsilon$ is the predictive state space
\end{itemize}

Using the options framework \cite{sutton1999} to select action possibilities is a well-known approach in RL.
An advantage of using the options framework is it provides a way to predict the outcome of composed options, i.e. execution of several options in sequence, which is analogous to composed affordances.
The second approach is a little more nuanced in that the original MDP, which may be partially observable \cite{schaul2013}, is transformed into a modified MDP $M^{\Upsilon}$ given by tuple $(\Upsilon, A, P^{\Upsilon}, r, \gamma)$ where $\Upsilon$ is the predictive state space and $P^{\Upsilon}$ is the transition probabilities in the predictive state space, i.e. $p(\upsilon_{t+1}|a_{t},\upsilon_{t})$.
In this modified MDP setting, a policy $\pi(a|\upsilon)$ is learned which maximizes future accumulated reward, i.e. $\pi = arg\,max_{\pi}{\sum_{k=0}^{\infty}{\gamma^k r_{t+k+1}}}$.
The potential advantages of maximizing reward in $M^{\Upsilon}$ versus $M$ are

\begin{itemize}
\item $\upsilon \in \Upsilon$ may be a very compact representation of state \cite{littman2002} \cite{schaul2013}
\item Faster learning in complex, high dimensional environments
\item Policies choose primitive actions rather than selecting temporally extended options which may be challenging to learn
\end{itemize}

\subsection{More Research is Needed}
% TODO: Move this section to the end of the paper and focus on only a few very important topics
% TODO: If possible highlight examples of the issue and why this topic is important for further research
There are many open questions of research that need to be addressed to fully utilize the proposed computational framework of affordances in real-world robotics.
A list of some of the important research questions are provided:

\begin{itemize}
\item How to learn a predictive state representation, especially in partially observable environments? \cite{schlegel2018} \cite{schaul2013}
\item What kind of predictions can we learn? \cite{deasis2018}
\item How to learn a hierarchy of options and predictions to learn behavior that affords behavior? \cite{sutton1999}
\item How to learn very long-term predictions with discount values very close to $1$? \cite{romoff2019}
\item How to improve off-policy learning with deep networks, especially with constrained behavior policies for safe and minimal exploration \cite{fuimoto2018}
\item How to achieve robust control with a predictive state representation? \cite{graves2019a} \cite{graves2020}
\end{itemize}

The long term challenge with affordances and predictive state representations is learning to discover the predictive questions.
This includes learning (1) the options, (2) the cumulants, (3) the GVFs or affordances, and (4) the predictive state representation as numbered in Figure \ref{fig_affordances}.
Learning a predictive state representation (PSR) is important for finding utility in GVFs in robotics; without a state representation, where the probability of observing the next state is only dependent on the current state and action taken, integrating GVF predictions into control algorithms may be a challenge.
\cite{schlegel2018} demonstrated that it is possible to learn state in partially observable environments with the right set of GVF predictions; they are easier to train and perform better than recurrent neural networks which remember a history of observations.
However, learning the GVF question is still an important area of research; this is commonly called the GVF discovery problem.
The predictive state learning algorithm must discover the (1)  cumulant $c$, (2) target policy $\tau$, and (3) termination function $\gamma$.
Options discovery, or skill discovery, can potentially be adapted for GVFs discovery since these approaches focus on learning options \cite{eysenbach2018} \cite{gregor2016} \cite{thomas2017} \cite{achiam2018} \cite{thomas2018} \cite{machado2017} \cite{harutyunyan2019}.
However, more work is needed to scale up option discovery to complex environments and learn a useful skill set that enables solving many problems including complex sequential tasks.
Establishing a good objective function for learning state with a collection of GVFs is an important challenge in this domain.

Understanding what kind of predictions we can learn with GVFs is an important problem to help us understand their flexibility and limitations.
For example, authors in \cite{deasis2018} introduced a way to predict coefficients of a discrete Fourier transform (DFT) at any desired frequency of the cumulant time series using complex-valued discount values.
Predicting many of these Fourier coefficients at different frequencies allows for the prediction of not just a future sum of cumulants but potentially an entire sequence of future cumulants through an inverse Fourier transform.

Composing predictions is important for planning in more complex environments and problems to be able to predict the long term outcome of following more than one option in sequence where the next option begins following termination of the previous option.
In affordance literature this is called compositional affordances.
Extending GVFs to compositional GVFs is a trivial extension of the options framework \cite{sutton1999} where the options framework provides the mathematical tools and theories for learning these kinds of predictions.
A key challenge though is how to learn what options to predict in sequence; this is a combinatorial problem that explodes with the number of options, or skills, available to the agent.

There are two additional challenges with learning GVFs with deep neural networks: (1) off-policy stability, and (2) managing inductive biases.
For the first problem, if the behavior policy is too constrained, the importance sampling ratio to correct for the behavior policy may be very large and even infinite.
This can create stability challenges when learning GVFs with any function approximation method: most notably deep neural networks.
For the second problem, if the behavior policy fails to visit large parts of the state space, the function approximation must focus on managing the inductive biases for generalizing to unseen states.

The final challenge is improving the data efficiency of learning GVFs with deep neural networks.
This challenge also exists in supervised learning; however, in deep reinforcement learning it is exacerbated by collecting data online while updating the policy used to collect the data.
Traditionally when learning GVFs, the policy is defined in advanced and therefore fixed; this allows the predictions to learn comparatively quickly.
However, when learning the policies through GVF prediction discovery, the policies are changing and this can further harm the data efficiency.

Having many predictions about the outcomes of different policies can be used for planning as a way to select policies based on their anticipated outcomes.
The expected outcome for a policy is the prediction of future accumulated cumulant for that policy, i.e. a GVF.
Control can be achieved by selecting a policy (or sequence of policies) from among the predictions of anticipated outcomes, or affordances.
However, the challenge is achieving robust control where (1) predictions are being continually learned and improved over time, (2) environments are highly dynamic and complex, and (3) environment is partially observable.

An alternative to learning control behavior is to leverage classical control theory with predictive state representations.
Specifically, one could evaluate a cost function of the set of expected future outcomes (accumulated cumulants) and choose predictions amoung the different policies.
